Uniformity of point samples in metric spaces using gap ratio

Teramoto et al. defined a new measure called the gap ratio that measures the uniformity of a finite point set sampled from $\cal S$, a bounded subset of $\mathbb{R}^2$. We generalize this definition of measure over all metric spaces by appealing to covering and packing radius. The definition of gap ratio needs only a metric unlike discrepancy, a widely used uniformity measure, that depends on the notion of a range space and its volume. We also show some interesting connections of gap ratio to Delaunay triangulation and discrepancy in the Euclidean plane. The major focus of this work is on solving optimization related questions about selecting uniform point samples from metric spaces; the uniformity being measured using gap ratio. We consider discrete spaces like graph and set of points in the Euclidean space and continuous spaces like the unit square and path connected spaces. We deduce lower bounds, prove hardness and approximation hardness results. We show that a general approximation algorithm framework gives different approximation ratios for different metric spaces based on the lower bound we deduce. Apart from the above, we show existence of coresets for sampling uniform points from the Euclidean space -- for both the static and the streaming case. This leads to a $\left( 1+\epsilon \right)$-approximation algorithm for uniform sampling from the Euclidean space.

==> genmet.tex <==
\section{A General Approximation Hardness Result}
\label{sec:genmet}
%\vspace{-.12in}
In this section, we show that the gap ratio problem is hard to approximate within a factor of $2$ for a general metric space.  
%\vspace{-.08in}
\begin{theo}\label{theo:genmet}
In a general metric space, it is NP-hard  to approximate the gap ratio better than a factor of 2.
\end{theo}
%\vspace{-.18in}
\begin{ourproof}
To show this hardness, we make a reduction from independent dominating set problem, where the dominating set is also independent set. This problem is known to be NP-hard \cite{Garey:1990:CIG:574848}. The independent dominating set problem statement is as follows. Given a graph $G$ and and integer $k<|V|$ does there exist a set $D$ of size at most $k$ such that $D$ is a dominating set as well as an independent set.

Let $G=\left(V,E\right)$ and $k$ be an instance of independent domination problem. We make a weighted complete graph over $V$ such that all edges present in $G$ have weight $1$ and all other edges have weight $2$. Now the metric space $\cal M$ is given by the vertex set of the complete graph and the metric is defined by the edge weights. 

We now show that $G=(V,E)$ has an independent dominating set of cardinality $k$ if and only if there exists a sampled set $P$ in $\mathcal{M}$ of $k$ points with gap ratio $1$. Let $D$ be an independent dominating set of $G$ of cardinality $k$. Let the sampled set $P$ in $\mathcal{M}$ is given by $P=D$. Now since $D$ is independent in $G$, any two points in $P$ are at a distance of $2$ in the metric space $\mathcal{M}$. Thus $r=1$. Since $D$ is a dominating set of $G$, every point in $\cal M$ has an edge of weight $1$ with some point in $P$. Thus $R=1$. Hence, the gap ratio equals $1$.

Conversely, suppose a point set $P$ of cardinality $k$ has been selected from $\cal M$ such that the gap ratio is $1$. Note that in the metric space, the value of $R$ is either $1$ or $2$ and the value of $r$ is either $\frac{1}{2}$ or $1$. Consequently, the minimum gap ratio is $1$ and the only way that can happen is if $R$ and $r$ both take value $1$.
Now $R=1$ means the farthest point in $\cal M$ is at a distance of $1$ from the set $P$. Thus every point in $\cal M$ has an edge of weight $1$ with some point in $P$ or is in $P$. Thus $P$ forms a dominating set in $G$. Also, as $r=1$, we have the closest pair in $P$ is distance $2$ apart. Thus, the set $P$ is an independent dominating set in $G$ of cardinality $k$.
\end{ourproof}

%Suppose, for a contradiction, there is an $\alpha$-approximation algorithm for the gap ratio problem, where $\alpha<2$. Since the minimum value of the gap ratio is $1$, we can have a set $P$ of cardinality $k$ in $\cal M$ with a gap ratio $\alpha\times1<2$. Also note that, the possible values of gap ratio are $1$, $2$, and $4$. Hence, $P$ must have gap ratio $1$. From the above claim, we have an independent dominating set of cardinality $k$ of the underlying graph $G$.
%\end{ourproof}
%\vspace{-.28in}
